En route to Background Independence: Broken split-symmetry, and how to restore it with bi-metric average actions

The most momentous requirement a quantum theory of gravity must satisfy is Background Independence, necessitating in particular an ab initio derivation of the arena all non-gravitational physics takes place in, namely spacetime. Using the background field technique, this requirement translates into the condition of an unbroken split-symmetry connecting the (quantized) metric fluctuations to the (classical) background metric. If the regularization scheme used violates split-symmetry during the quantization process it is mandatory to restore it in the end at the level of observable physics. In this paper we present a detailed investigation of split-symmetry breaking and restoration within the Effective Average Action (EAA) approach to Quantum Einstein Gravity (QEG) with a special emphasis on the Asymptotic Safety conjecture. In particular we demonstrate for the first time in a non-trivial setting that the two key requirements of Background Independence and Asymptotic Safety can be satisfied simultaneously. Carefully disentangling fluctuation and background fields, we employ a `bi-metric' ansatz for the EAA and project the flow generated by its functional renormalization group equation on a truncated theory space spanned by two separate Einstein-Hilbert actions for the dynamical and the background metric, respectively. A new powerful method is used to derive the corresponding renormalization group (RG) equations for the Newton- and cosmological constant, both in the dynamical and the background sector. We classify and analyze their solutions in detail, determine their fixed point structure, and identify an attractor mechanism which turns out instrumental in the split-symmetry restoration. We show that there exists a subset of RG trajectories which are both asymptotically safe and split-symmetry restoring. We conclude that the next generation of truncations must be bi-metric.

==> Definitions.tex <==
\makeatletter
\renewcommand*\env@matrix[1][*\c@MaxMatrixCols c]{%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{#1}}
\makeatother

\makeatletter
\def\hlinewd#1{%
\noalign{\ifnum0=`}\fi\hrule \@height #1 %
\futurelet\reserved@a\@xhline}
\makeatother

\renewcommand{\epsilon}{\varepsilon}

\newcommand{\sP}[2]{\left(#1,#2\right)}
\newcommand{\fsp}{\mathds{F}_{\Phi}}
\newcommand{\makeNote}{\marginpar[\hfill \color{red} $\longrightarrow$]{\color{red}$\longleftarrow$\hfill}}
\newcommand{\sM}{\mathcal{G}[\bar{\Phi}]}
\newcommand{\sMg}{G[\bar{\Phi}]}

\renewcommand{\vec}[1]{\boldsymbol{#1}}

\newcommand{\vfb}{V}

%Reference-Punkte
\newcommand{\refpoint}[3]{\begingroup \begin{parcolumns}[colwidths={1=0.3cm},nofirstindent=true]{2}\colchunk{}%
\colchunk{ \raggedright {\sffamily \bf \fontsize{12pt}{12pt}\selectfont #2 }\\ {\rmfamily \fontsize{12pt}{12pt}\selectfont \hspace{0.05cm} #1 \, , \, \cite{#3}.}\linebreak } \end{parcolumns}\endgroup}
\newcommand{\RegA}{R}


\newcommand{\cix}{I}

%Cutoff-Operator
\newcommand{\CutO}{{\cal R}}
\newcommand{\CutM}{R}


% \newcommand{\iou}[2]{\genfrac{(}{)}{0pt}{3}{\mkern-3mu#1\mkern-2.5mu}{\mkern-3mu#2\mkern-2.5mu}}
 \newcommand{\iou}[2]{{\scriptscriptstyle \underline{\bm{(}\mkern-1.5mu#1;#2\bm{)}\mspace{-3.0mu}}\mspace{3.0mu}}}
\newcommand{\ivC}[1]{\mspace{-1.5mu}\underline{\boldsymbol{#1}\mspace{-3.0mu}}\mspace{3.0mu}}
\newcommand{\ivc}[2]{\ivC{#1}}
\newcommand{\basisSet}{{\cal B}}
\newcommand{\be}[2]{e_{\iou{#1}{#2}}}
\newcommand{\bE}[2]{E_{\,\ivc{#1}{#2}}}
\newcommand{\bEi}[2]{E_{\iou{#1}{#2}}}
\newcommand{\bEp}[3]{E^{\mSE(#3)}_{\ivc{#1}{#2}}}
\newcommand{\bEpi}[3]{E^{\mSE(#3)}_{\iou{#1}{#2}}}
% \newcommand{\bE}{E}
 \newcommand{\ip}[3]{\left(#1 | #2 \right)_{#3}}

%roman numbers
\makeatletter
\newcommand{\rmnum}[1]{\romannumeral #1}
\newcommand{\Rmnum}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

%Textbausteine im Mathemodus

\newcommand{\arbit}{\text{arbitrary}}
\newcommand{\selfcon}{\text{selfcon}}


%###############################################################################
%    MATHEMATIK
%###############################################################################
 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Zahlenbereiche & Räume
\newcommand{\noR}{\mathds{R}}
\newcommand{\noN}{\mathds{N}}
\newcommand{\noC}{\mathds{C}}
\newcommand{\noZ}{\mathds{Z}}
\newcommand{\Hoe}[2]{C^{#1 , #2}} %Hoelder-Raum
\newcommand{\SteC}[1]{C^{#1}}
\newcommand{\Tens}[3]{\mathcal{T}^{#1}_{#2}{(#3)}}
\newcommand{\On}[1]{O(#1)}
\newcommand{\SOn}[1]{SO(#1)}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Differential-Geometrie
\newcommand{\Lie}{\mathscr{L}}  %Lie-Ableitung
\newcommand{\MaF}{\mathcal{M}} %Integrations-Riemann-Mannigfaltigkeit
\newcommand{\bsl}{\backslash}
%g-bar
\newcommand{\MaFs}{\mathcal{M}}  %Allgemeine Riemann-Mannigfaltigkeit
\newcommand{\MIF}{\mathcal{N}_{\hyp}}
\newcommand{\SymSet}{\text{Sym}[\Tens{0}{2}{\MaFs}]}
\newcommand{\SymSets}{\text{Sym}}
\newcommand{\TM}{\mathcal{T}}  %tangential space
\newcommand{\VF}{\mathscr{T}^1_0} %space of vectorfields
\newcommand{\coDif}{\updelta}
\newcommand{\Dif}{\text{d}}
\newcommand{\Indx}{\text{\tiny index}}
\newcommand{\Hstar}{\star}
\newcommand{\kForm}[2]{\stackrel{\text{\tiny #2}}{#1}\,}
\newcommand{\harmF}{\mathcal{H}}
\newcommand{\sym}[1]{\text{sym}\left[#1\right]}
%\newcommand{\Lie}[1]{\mathscr{L}_{#1}}
\newcommand{\LieBra}[2]{\left[#1;#2\right]_{\mathscr{L}}}
\newcommand{\tp}{\mathcal{T}}
\newcommand{\mx}{\mathcal{X}}
\newcommand{\vecSp}{X}
\newcommand{\TgSp}[2]{T_{#2} #1}
\newcommand{\TSp}[1]{T #1}
\newcommand{\atlas}{\mathcal{A}}
\newcommand{\Christ}[3]{\left\{\genfrac{}{}{0pt}{1}{#1}{#2\, #3}\right\} }

 
 
\newcommand{\LFT}[1]{\text{LFT}\left\{#1\right\}}
\newcommand{\txLFT}{{\bf LFT }}
\newcommand{\LT}[1]{\text{LT}\left\{#1\right\}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Geometrische Objekte
\newcommand{\LaB}{\Box}    %Laplace-Beltrami operator
\newcommand{\Ric}{R}     % Ricci tensor
\newcommand{\Rm}{R}     % Riemann tensor
\newcommand{\SR}{R}     % Scalar curvature
\newcommand{\EinT}{G}    %Einstein tensor
\newcommand{\bEinT}{\bar{G}}   %Einstein tensor bar
\newcommand{\Ricb}{\bar{\Ric}}     % Ricci tensor
\newcommand{\Rmb}{\bar{\Rm}}     % Riemann tensor
\newcommand{\SRb}{\bar{\SR}}     % Scalar curvature
\newcommand{\Z}{D}      % connection
\newcommand{\ZH}{\text{D}}      % connection
\newcommand{\CoC}[3]{\Gamma_{#2 #3}^{#1}}  %Connection Coefficient}
\newcommand{\CoCbar}[3]{\overline{\Gamma}_{#2 #3} ^{#1}} %Connection
%Coefficient}
\newcommand{\CoCA}[6]{\widetilde{\Gamma}_{\text{g}}\left[#5\right]_{#2 #3} ^{#1}} %general
%Connection Coefficient}
\newcommand{\Cris}[4]{\frac{1}{2} g^{#1 #4} \left(\partial_{#2}g_{#4
#3}+\partial_{#3}g_{#2 #4}-\partial_{#4}g_{#2 #3}\right)}
\newcommand{\CrisA}[7]{\frac{1}{2} #5^{#1 #4} \left(#7_{#2}#6_{#4
#3}+#7_{#3}#6_{#2 #4}-#7_{#4}#6_{#2 #3}\right)}
\newcommand{\bg}{\bar{g}}   %Metric
\newcommand{\bZ}{\bar{\Z}}   %Connection
\newcommand{\bgm}{\bg}
\newcommand{\flH}{\hat{h}}		%fluctuation metric 
\newcommand{\hb}{\bar{h}}
\newcommand{\hx}{h}
\newcommand{\hhat}{\tilde{h}}   %traceless part of h
\newcommand{\htr}{\phi}
%transversal-traceless part
%------------------------------------------------------------------------------
%Oberflaeche
\newcommand{\iM}{H}  %induzierte Metrik auf der Oberfläche
\newcommand{\EC}{K}  % extrinsic curvature
%------------------------------------------------------------------------------
%GeometryOnSurface kapitel
\newcommand{\hyp}{\mathcal{H}}		%hyperplane
\newcommand{\derMat}{B}		%deformation matrix
\newcommand{\matA}{A}		%orthogonal matrix
\newcommand{\tM}{\tilde{t}}		%transverse metric
%------------------------------------------------------------------------------
%Critical Hypersurface
\newcommand{\stabM}{B}
\newcommand{\cUV}{\mathscr{S}_{\text{UV}}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Funktions Definitionen
\newcommand{\id}{\delta} % Identity
\newcommand{\idm}{\Eins} % Identity
\newcommand{\var}{\delta} %variation
\newcommand{\com}[2]{\left[#1,#2\right]} % commutator
\newcommand{\varFunc}{\delta}     %functional derivative
%symbol
\newcommand{\fD}[2]{\frac{\varFunc #1}{\varFunc #2}} % functional derivative
\newcommand{\fDn}[3]{\frac{\varFunc^{#3} #1}{\varFunc #2}} %functional nth
%derivative
\newcommand{\sgn}{\text{sgn}}  %signum
\newcommand{\adj}{\,\text{adj}}  %adjoint
\newcommand{\tr}{\text{tr}}   %trace
\newcommand{\Tr}{\text{Tr}}   %functional Trace
\newcommand{\Order}[1]{\mathcal{O}(#1)}  %Ordnung
\newcommand{\OrderX}[2]{\mathcal{O}^{#2}(#1)}
\newcommand{\epsTen}{\varepsilon}						%{{\Large\text{$\upvarepsilon$}}}
\newcommand{\GF}[1]{\Gamma\left(#1\right)}   %Gamma-function
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Differentialoperatoren
\newcommand{\Quabla}{\hbox{\footnotesize{$\Box$}}} % D'Alembert
\newcommand{\Laplace}{\Delta}
\newcommand{\Ellipt}{\Delta_E}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Integration
\newcommand{\IntSp}[2]{\int \md^{#1} #2 \,} %spacetime-integral dimension #1
\newcommand{\IntSpI}[2]{\int^{#1}_{#2} }  %spacetime-integral
%dimension #1
\newcommand{\IntSpM}[3]{\int_{#3} d^{#1} #2 \,} %spacetime-integral dimension #1
%restricted on #3
\newcommand{\IntSpMs}[3]{\int^{#2}_{#3}} %spacetime-integral dimension #1
\newcommand{\PI}{\mathcal{PI}}   %partielle Integration
\newcommand{\md}{\text{d}}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Distribution
\newcommand{\DisD}[1]{\delta\left(#1\right)}  %Delta Distribution
\newcommand{\DisDr}[1]{\delta\left[#1\right]}  %Delta Distribution of Functionals
\newcommand{\kDelta}{\delta}
\newcommand{\Heaviside}[1]{\Theta \left(#1\right)}
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%HILFSDEFINITIONEN
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Allgemeine Symbole
\newcommand{\Ii}{\mathrm{i}}      
%imaginary number
\newcommand{\LHS}{\text{LHS}}     
%LHS
\newcommand{\RHS}{\text{RHS}}     
%RHS
\newcommand{\QED}{\begin{flushright} \color{Text} $\Box$ \end{flushright}}
%q.e.d.
\newcommand{\Res}{\text{Res}}     
%Residium
\newcommand{\xfrac}[2]{%     
%Bruch mit schrägstrich
\mbox{\raisebox{0.4ex}{\ensuremath{\displaystyle #1}\hspace{0.2ex}}%
{\raisebox{-0.1ex}{\Large /}}%
\raisebox{-0.2ex}{\ensuremath{\displaystyle #2}}%
}%
}
\newcommand{\const}{\text{const}}    

 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Physikalische Objekte
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
%-------------------------------------------------------------------------------
%Wirkung
 
\newcommand{\SW}{S}  %Action
\newcommand{\ISW}{{\cal I}} 	%Integral part of Action 
\newcommand{\EA}{\Gamma}
\newcommand{\EAA}{\Gamma}  %Effective Average action
\newcommand{\CGF}{W}   %connected generating funcntional
\newcommand{\La}{\mathcal{L}}  %range density
\newcommand{\ParF}{\text{Z}}  %Partition function
 \newcommand{\ParFD}{\mathds{Z}}  %Partition function
 \newcommand{\frEny}{F}				%{\mathds{F}} 
%-------------------------------------------------------------------------------
%Felder
 
\newcommand{\Gh}{C}   %Ghost Faddeev-Popov
\newcommand{\GhA}{\bar{C}}  % Anti-Ghost
\newcommand{\Ghx}{\xi}   %Expectation Ghost Faddeev-Popov
\newcommand{\GhAx}{\bar{\xi}}  %Expectation Anti-Ghost
 
 
%-------------------------------------------------------------------------------
%Kosmologische Konstante
 
\newcommand{\CosmConst}{\lambda}
%
\newcommand{\Kk}{\CosmConst}  %Kosmologische Konstante (dim-less)
\newcommand{\Kkbar}{\Lambda}  % bare cosmological constant

\newcommand{\cf}{\Omega}

\newcommand{\KkbartD}{\Kkbar^{\dyn}}
\newcommand{\KkbarD}{\Kkbar_k^{\dyn}}  % bare cosmological constant
\newcommand{\KkbarB}{\Kkbar_k^{\background}}  % bare cosmological constant
%Surface
\newcommand{\KkEC}{\CosmConst^{\partial}}  %Kosmologische Konstante
% (dim-less) dM
\newcommand{\KkbarEC}{\bar{\CosmConst}^{\partial}}  % bare
%cosmological constant dM

\newcommand{\Kka}{\CosmConst_{1;k}}  %Kosmologische Konstante (dim-less)
\newcommand{\Kkb}{\CosmConst_{2;k}}  %Kosmologische Konstante (dim-less)
\newcommand{\KkECa}{\CosmConst^{\partial}_{1;k}}  %Kosmologische Konstante (dim-less)
\newcommand{\KkECb}{\CosmConst^{\partial}_{2;k}}  %Kosmologische Konstante (dim-less)
 
%-------------------------------------------------------------------------------
%Newtonskonstante

\newcommand{\Nkpd}{\text{g}^{\dyn \dotpart}}  %Newtons Konstante (dim-less)
\newcommand{\Nkd}{\text{g}^{\dyn}}  %Newtons Konstante (dim-less)
\newcommand{\Nk}{G}  %Newtons Konstante 
\newcommand{\Nkbar}{\Nk_N}%{\overline{\text{G}}} %Newtons Konstante bar
%Surface
\newcommand{\NkECd}{\text{g}^{\dyn,\partial}}  %Newtons Konstante
%dim-less
\newcommand{\NkEC}{G^{\partial}}  %Newtons Konstante 
\newcommand{\NkbarEC}{\overline{G}} %Newtons Konstante bar
 
%-------------------------------------------------------------------------------
%Konstanten
 
\newcommand{\kap}{\kappa}
\newcommand{\kapEC}{\kappa}
%
\newcommand{\CcM}{C_{M}}  %C_V constante p.18 M.R.
\newcommand{\CcT}{C_{\hhat}}  %C_T constante p.17 M.R.
\newcommand{\CcS}{C_{\htr}}  %C_S constante p.17 M.R.
%
\newcommand{\CHyp}{\varpi}%C_{\text{Hyp}}}
 
%-------------------------------------------------------------------------------
%Funktionen
 
%Treshold
\newcommand{\Thrf}[5]{\Phi^{#1 ; #3}_{#2}\left(#4,#5\right)}
%Threshold-function
\newcommand{\ThrfA}[3]{\Phi^{#1}_{#2}\left({\scriptstyle #3}\right)}
\newcommand{\ThrfAn}[4]{\Phi^{#1\,{\scriptscriptstyle (0,#4,0)}}_{#2}\left({\scriptstyle #3}\right)}
\newcommand{\ThrfBn}[4]{\widetilde{\Phi}^{#1\,{\scriptscriptstyle (0,#4,0)}}_{#2}\left({\scriptstyle #3}\right)}
\newcommand{\qA}[3]{q^{#1}_{#2}\left({\scriptstyle #3}\right)}  
\newcommand{\qAn}[4]{q^{#1\,{\scriptscriptstyle (0,#4,0)}}_{#2}\left({\scriptstyle #3}\right)}  
%Threshold-function
\newcommand{\ThrfB}[3]{\widetilde{\Phi}^{#1}_{#2}\left({\scriptstyle #3}\right)}
%Threshold-function
\newcommand{\GThrf}[5]{\Upsilon^{#1 ; #3}_{#2}\left(#4,#5\right)}
%generalized Threshold-function
\newcommand{\GThrfA}[4]{\Upsilon^{#1}_{#2 ; #4}\left(#3\right)} 
%generalized Threshold-function
\newcommand{\GThrfB}[4]{\widetilde{\Upsilon}^{#1}_{#2 ; #4}\left(#3\right)} 	
%generalized Threshold-function
%Trace-Abbreviations
\newcommand{\Af}{\mathcal{A}}
\newcommand{\Nf}{\mathcal{N}}
%
\newcommand{\BTfA}[1]{B_{\Phi}\left(#1 \right)}
\newcommand{\BTfB}[1]{B_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\BTfAEC}[1]{B^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\BTfBEC}[1]{B^{\partial}_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\DTfA}[1]{b_{\Phi}\left(#1 \right)}
\newcommand{\DTfB}[1]{b_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\DTfAEC}[1]{b^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\DTfBEC}[1]{b^{\partial}_{\widetilde{\Phi}}\left(#1 \right)}
%Bimetric
\newcommand{\BBTfA}[1]{\overline{B}_{\Phi}\left(#1 \right)}
\newcommand{\BBTfB}[1]{\overline{B}_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\BBTfAEC}[1]{\overline{B}^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\BBTfBEC}[1]{\overline{B}^{\partial}_{\widetilde{\Phi}}
\left(#1\right)}
\newcommand{\BDTfA}[1]{\overline{b}_{\Phi}\left(#1 \right)}
\newcommand{\BDTfB}[1]{\overline{b}_{\widetilde{\Phi}}\left(#1 \right)}
\newcommand{\BDTfAEC}[1]{\overline{b}^{\partial}_{\Phi}\left(#1 \right)}
\newcommand{\BDTfBEC}[1]{\overline{b}^{\partial}_{\widetilde{\Phi}}\left(#1\right)}
%
\newcommand{\CDel}[2]{\text{c}_{#1}^{#2}}
%Mass-Dimension
\newcommand{\Mdim}[1]{\left[#1\right]}  %mass-dimension
 
%-------------------------------------------------------------------------------
%Bimetric


\newcommand{\ph}{{\scriptscriptstyle \#}}
\newcommand{\agf}{\hat{\alpha}}
\newcommand{\ags}{\hat{\alpha}^{\text{new}}}

\newcommand{\sRM}{\text{Riem}}

\newcommand{\DThrfA}[3]{\zeta^{#1\,(#3)}_{#2}}
% \newcommand{\rhoN}{\rho_{\text{grav}}}
\newcommand{\rhoN}{}
\newcommand{\rhoG}{\rho_{\text{gh}}}
\newcommand{\rhoGk}{\rho_{\text{gh}\,k}}
\newcommand{\rhoP}{\rho_{\text{P}}}
\newcommand{\rhoD}{\rho_{\text{D}}}
\newcommand{\rhoA}{\gamma}
 
\newcommand{\background}{\text{B}}
\newcommand{\dyn}{\text{Dyn}}
\newcommand{\lin}{\text{lin}}
\newcommand{\sm}{\text{sm}}
 \newcommand{\bM}{\text{bm}}
%

\newcommand{\zh}{A}

\newcommand{\KkB}{\CosmConst^{\background}}  %Kosmologische Konstante
\newcommand{\KkD}{\CosmConst^{\dyn}} %Kosmologische Konstante
% (dim-less)
\newcommand{\KkECB}{\CosmConst^{\partial}_{\background , k}}
%Kosmologische Konstante  (dim-less) dM
% \newcommand{\KkbarB}{\bar{\CosmConst}_{2;k}}
\newcommand{\KkbarBEC}{\bar{\CosmConst}_{2;k}^{\partial}}
%
\newcommand{\ZfacD}{Z^{\dyn}_{k}}
\newcommand{\ZfacGB}{Z^{\background}_{k}}
%
\newcommand{\ZfacB}{Z^{\background}_{k}}
\newcommand{\ZfacBEC}{Z^{\partial}_{2,k}}
%
\newcommand{\ZfacBt}{Z_{k}}
\newcommand{\ZfacBtEC}{Z^{\partial}_{k}}
%
\newcommand{\NkbarB}{\overline{G}^{\background}} %Newtons Konstante bar
 
\newcommand{\NkdB}{\text{g}^{\background}}  %Newtons Konstante
% (dim-less)
%
\newcommand{\NkbarECB}{\overline{G}^{\background}}
\newcommand{\NkECdB}{\text{g}^{\background,\partial}}  %Newtons
% Konstante dim-less
%
\newcommand{\biM}{\bar{\iM}}
\newcommand{\bEC}{\bar{\EC}}
%
\newcommand{\aDzB}{\eta_2}  %anomalous dimension
\newcommand{\aDzECB}{\eta_2^{\partial}}
 
%-------------------------------------------------------------------------------
%Regulator
 
\newcommand{\RegGr}{R^{\text{grav}}} %Regulator grav
\newcommand{\RegGn}{R} %Regulator grav
\newcommand{\RegGh}{R^{\text{gh}}} %Regulator ghost
\newcommand{\RegX}[1]{R^{(0)}\left(#1\right)} %regulator R0
\newcommand{\RegXd}[1]{R^{(0)\prime}\left(#1\right)} %regulator R0 deriv
\newcommand{\RegY}[2]{R_{\text{#2}}^{(0)}\left(#1\right)} %regulator R0
\newcommand{\RegXdot}[1]{\dot{R}^{(0)}\left(#1\right)}
\newcommand{\RegO}{\RegX{\tfrac{-\bZ^2}{k^2}}} %regulator R0
\newcommand{\RegOd}{\RegXd{\tfrac{-\bZ^2}{k^2}}} %regulator R0 partal diff
\newcommand{\RegOpt}{R_{\text{opt}}} %regulator R0
 
%-------------------------------------------------------------------------------
%

\newcommand{\dEps}{\boldsymbol{\delta}^{\text{split}}_{\epsilon}}
% \newcommand{\dEps}{\dEp^{\text{{\bf split}}}}
\newcommand{\dBgt}{\boldsymbol{\delta}^{\text{{B}}}_{v}}

\newcommand{\kA}{A^{\background}}
\newcommand{\kAx}{A^{\cix}}

\newcommand{\kB}{B_1^{\background}}

\newcommand{\kAD}{B_1^{\dyn}}
\newcommand{\kBD}{B_2^{\dyn}}

\newcommand{\dBb}{B_2^{\dyn}}
\newcommand{\dBa}{B_1^{\dyn}}

\newcommand{\bmA}{\mathcal{B}_{11}}
\newcommand{\bmB}{\mathcal{B}_{12}}
\newcommand{\bmC}{\mathcal{B}_{21}}
\newcommand{\bmD}{\mathcal{B}_{22}}
\newcommand{\bmE}{\mathcal{B}_{31}}
\newcommand{\bmF}{\mathcal{B}_{32}}
\newcommand{\bmG}{\mathcal{B}_{41}}
\newcommand{\bmH}{\mathcal{B}_{42}}
\newcommand{\bmI}{\mathcal{B}_{43}}

\newcommand{\attr}{\bullet}
\newcommand{\AttrL}{\text{{\bf (Attr)$^{\background}$}}}
\newcommand{\SolAttr}{\text{Sol}_{\attr}^{\background}}
\newcommand{\fpnD}{{\bf NG$_+^{\dyn}$}}
\newcommand{\fpnDn}{{\bf NG$_-^{\dyn}$}}

\newcommand{\fpgD}{{\bf G$^{\dyn}$}}
\newcommand{\fpnB}{{\bf NG$_+^{\background}$}}
\newcommand{\fpnBn}{{\bf NG$_-^{\background}$}}
\newcommand{\fpgB}{{\bf G$^{\background}$}}

\newcommand{\fpnO}{{\bf NG$_+^{(0)}$}}
\newcommand{\fpgO}{{\bf G$^{(0)}$}}

\newcommand{\fpnBO}{{\bf NG$_+^{\background\slash(0)}$}}
\newcommand{\fpgBO}{{\bf G$^{\background\slash(0)}$}}



\newcommand{\fpC}{{$\oplus$}}
\newcommand{\fpL}{{\bf FP}}

\newcommand{\Prohtr}{P_{\htr}}  % Projector htrace
\newcommand{\Prohhat}{P_{\hhat}} % Projector hhat
 
\newcommand{\ZfacG}{Z_{k}}
\newcommand{\ZfacECG}{Z^{\partial}_{k}}
\newcommand{\NkdG}{\text{g}}
 
\newcommand{\NkECdG}{\text{g}^{\partial}}
\newcommand{\aDzG}{\eta}
 
\newcommand{\aDz}{\eta^{\dyn}}  %anomalous dimension
\newcommand{\Zfac}{Z_{1,k}}
 
 
\newcommand{\aDzEC}{\eta^{\partial} _{\text{N}}}  %anomalous
% dimension
\newcommand{\ZfacEC}{Z^{\partial}_{1,k}}
 
\newcommand{\dotpart}{\cdot \slash \partial}
\newcommand{\IR}{IR }
\newcommand{\UV}{UV }
 
%-------------------------------------------------------------------------------
%MATTER INDUCED Variables
 
\newcommand{\PotA}{V(A)}
\newcommand{\PotAk}{V_k(A)}
\newcommand{\PotAkA}{V^{(0)}_k(A)}
\newcommand{\PotAkB}{V^{(1)}_k(A)}
\newcommand{\PotAd}[1]{V^{#1}_k(A)}
\newcommand{\potAk}{v_k(A)}
% \newcommand{\tg}{\text{g}}
\newcommand{\tg}{g}
\newcommand{\tgD}{g^{\dyn}}
\newcommand{\tgB}{g}
\newcommand{\nkA}{G_k^{(0)}}
\newcommand{\nkD}{G_k^{\dyn}}
\newcommand{\nkbB}{G_k^{\background}}

\newcommand{\nkB}{G_k^{(1)}}
\newcommand{\kkA}{\Lambda_k^{(0)}}
\newcommand{\kkB}{\Lambda_k^{(1)}}
\newcommand{\polyn}[1]{\text{Polyn}(#1)}
\newcommand{\Nkbart}{G_N}
\newcommand{\Kkbart}{\Lambda}

 
 
%-------------------------------------------------------------------------------
%-------------------------------------------------------------------------------
%-------------------------------------------------------------------------------
\newcommand{\AS}{A^{\partial}} 

\newcommand{\EAAbulk}{\EAA^{\text{bulk}}}
\newcommand{\EAAS}{\EAA^{\partial}}
\newcommand{\flcb}{\bar{h}}
\newcommand{\FPop}{\mathcal{M}}
\newcommand{\ud}[2]{^{#1}_{\phantom{#1}#2}}
\newcommand{\du}[2]{_{#1}^{\phantom{#1}#2}}
\newcommand{\Id}{I}
\newcommand{\calE}{{\cal E}}

